Formation of the polar debris disc around 99 Herculis

We investigate the formation mechanism for the observed nearly polar aligned (perpendicular to the binary orbital plane) debris ring around the eccentric orbit binary 99 Herculis. An initially inclined nonpolar debris ring or disc will not remain flat and will not evolve to a polar configuration, due to the effects of differential nodal precession that alter its flat structure. However, a gas disc with embedded well coupled solids around the eccentric binary may evolve to a polar configuration as a result of pressure forces that maintain the disc flatness and as a result of viscous dissipation that allows the disc to increase its tilt. Once the gas disc disperses, the debris disc is in a polar aligned state in which there is little precession. We use three-dimensional hydrodynamical simulations, linear theory, and particle dynamics to study the evolution of a misaligned circumbinary gas disc and explore the effects of the initial disc tilt, mass, and size. We find that for a wide range of parameter space, the polar alignment timescale is shorter than the lifetime of the gas disc. Using the observed level of alignment of 3 deg. from polar, we place an upper limit on the mass of the gas disc of about 0.014 M_sun at the time of gas dispersal. We conclude that the polar debris disc around 99 Her can be explained as the result of an initially moderately inclined gas disc with embedded solids. Such a disc may provide an environment for the formation of polar planets.

==> RESPONSE.tex <==
RESPONSE: We thank the referee for the helpful report.  We have dealt with all of the concerns and we hope that the paper is now acceptable for publication.

Scientific Editor's Comments:

The abstract is too long and should be shortened during revision to under 250 words.

RESPONSE: We have shortened the abstract to under 250 words (waiting on Steve for this).


Reviewer's Comments:

The authors set out to investigate a likely formation scenario for the polar debris disc observed around 99 Herculis as the end product of a more moderately misaligned disc. A gas disc subject to dissipation will polar align around an eccentric binary for a wide range of initial conditions. The authors use SPH simulations and analytical theory to estimate the polar alignment timescale for different initial gas disc masses, inclination, and radial extent. They find that polar alignment is quick enough compared to the disc lifetime. They also estimate a maximum disc mass at the point of decoupling based on the current observed inclination. The paper is well written and provides a significant contribution. I recommend acceptance for publication in MNRAS after the following concerns have been addressed: 

1- Throughout the paper, the polar alignment timescale is compared to the disc lifetime set by gas dispersal. However, dust particles will experience various degrees of decoupling depending on their Stokes number. Even small, initially well coupled, dust will grow to higher St and decouple from the gas evolution. Requiring the disc to polar-align before dust can grow and a significant fraction decouples is a much tighter constrain than requiring the gas to polar align before dispersal, estimated to happen after a few Myrs. I understand that this analysis is beyond the scope of the paper, but I think this caveat needs to be highlighted in more prominent places in the paper (it is currently alluded to in the last sentence in section 5).

RESPONSE: We acknowledge that dust grains will grow to higher Stokes number and eventually decouple from the gas. The dust particles must be coupled to the gas disc to reach a polar arrangement. Otherwise, a misaligned disc of debris will undergo differentiated precession and lead to spherical distribution rather than a disc. Dust grains are not included in our simulations but the time at which they decouple from the disc provides a more stringent constraint on the required polar alignment timescale than the lifetime of the disc. We have highlighted this caveat in the Introduction, Section 5.1, and the Conclusions.

2- Figure 1: The caption misses to define the blue lines (presumably retrograde circulating orbits)

RESPONSE: We have fixed the caption by defining the blue lines which represent the retrograde circulating orbits. 

3- The simulation lifetimes in terms of binary orbits can be inferred to be 1000 binary orbits but needs to be stated explicitly. At the moment it’s only stated in section 4.5 that it’s increased to 1500 for the most extended disc case.

RESPONSE: In the second paragraph in section 4.1 we have stated explicitly the simulation lifetime, in binary orbits, for both the narrow and extended discs.
